HELENE: Hessian Layer-wise Clipping and Gradient Annealing for Accelerating Fine-tuning LLM with Zeroth-order Optimization

Fine-tuning large language models (LLMs) poses significant memory challenges, as the back-propagation process demands extensive resources, especially with growing model sizes. Recent work, MeZO, addresses this issue using a zeroth-order (ZO) optimization method, which reduces memory consumption by matching the usage to the inference phase. However, MeZO experiences slow convergence due to varying curvatures across model parameters. To overcome this limitation, we introduce HELENE, a novel scalable and memory-efficient optimizer that integrates annealed A-GNB gradients with a diagonal Hessian estimation and layer-wise clipping, serving as a second-order pre-conditioner. This combination allows for faster and more stable convergence. Our theoretical analysis demonstrates that HELENE improves convergence rates, particularly for models with heterogeneous layer dimensions, by reducing the dependency on the total parameter space dimension. Instead, the method scales with the largest layer dimension, making it highly suitable for modern LLM architectures. Experimental results on RoBERTa-large and OPT-1.3B across multiple tasks show that HELENE achieves up to a 20x speedup compared to MeZO, with average accuracy improvements of 1.5%. Furthermore, HELENE remains compatible with both full parameter tuning and parameter-efficient fine-tuning (PEFT), outperforming several state-of-the-art optimizers. The codes will be released after reviewing.

==> sections/related_work_main.tex <==
% \section{Related Work}
% Zeroth-order (ZO) optimization has gained traction due to its ability to achieve comparable results to full-parameter fine-tuning while offering significant memory savings. Notably, MeZO (Malladi et al., 2023) has been adapted to fine-tune language models (LMs), reducing memory usage during training. However, recent advancements, such as Gautam et al. (2024) and Jiang et al. (2024), have aimed to improve gradient estimation, though challenges remain in terms of convergence rates and efficiency.

% Second-order optimization methods, which leverage curvature information, have also been explored for fine-tuning large language models (LLMs). Although methods such as those proposed by Martens & Grosse (2015) and George et al. (2018) have shown promise, they face limitations due to computational overhead and hardware dependencies. Despite these efforts, first-order optimizers like Adam remain dominant for decoder-only LLMs, partly due to the complexities associated with Hessian computation. Recent work, such as Zhao et al. (2024), has attempted to integrate Hessian-based methods, though improvements in stability and efficiency are still needed.

% Additionally, gradient clipping has long been a standard technique for stabilizing LLM training, particularly in handling rare examples and large gradient fluctuations. HELENE advances this approach by introducing Hessian clipping, which addresses errors in Hessian approximation and helps stabilize the optimization process in second-order methods.

% This condensed version outlines the key approaches and challenges in optimization for LLM fine-tuning, particularly focusing on zeroth- and second-order methods, and highlights the advancements introduced by the HELENE method.

==> tables/non-differentiable.tex <==
\begin{table*}[t]
\centering
\setlength{\tabcolsep}{14pt} % 减小列间距
\small % 调小字体
\resizebox{\textwidth}{!}{
    \begin{tabular}{lcccccc}
    \toprule
    \multicolumn{1}{c}{Model} & \multicolumn{4}{c}{RoBERTa-large (350M)} & \multicolumn{1}{c}{OPT-1.3B} \\
    \multicolumn{1}{c}{Task} & \tf{SST-2} & \tf{SST-5} & \tf{SNLI} & \tf{TREC} & \tf{SQuAD} \\
    \midrule
    Zero-shot  &79.00  &35.50 &50.20 &32.00 &53.67 \\
    \mezo{}       &92.70 &48.90 &82.70 &68.60 & \\
    \helen{}      & & & & & \\
    
    \bottomrule
    \end{tabular}
}
    \caption{
        Experiments on non-differentiable optimization objectives. Helen and \mezo{} are evaluated with non-differentiable objectives. For classification tasks on SST-2, SST-5, SNLI, and TREC, RoBERTa-large is optimized with full parameters, and accuracy is measured on 500 examples. For SQuAD, OPT-13B is optimized with prefix tuning, and F1 score is evaluated on 1,000 examples.
    }
    \label{tab:non_differential}
\end{table*}

